FlowSearch: Advancing deep research with dynamic structured knowledge flow

Deep research is an inherently challenging task that demands both breadth and depth of thinking. It involves navigating diverse knowledge spaces and reasoning over complex, multi-step dependencies, which presents substantial challenges for agentic systems. To address this, we propose FlowSearch, a multi-agent framework that actively constructs and evolves a dynamic structured knowledge flow to drive subtask execution and reasoning. FlowSearch is capable of strategically planning and expanding the knowledge flow to enable parallel exploration and hierarchical task decomposition, while also adjusting the knowledge flow in real time based on feedback from intermediate reasoning outcomes and insights. FlowSearch achieves competitive performance on both general and scientific benchmarks, including GAIA, HLE, GPQA and TRQA, demonstrating its effectiveness in multi-disciplinary research scenarios and its potential to advance scientific discovery. The code is available at https://github.com/InternScience/InternAgent.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/bk.tex <==
% The abstract paragraph should be indented 1/2~inch (3~picas) on both left and
% right-hand margins. Use 10~point type, with a vertical spacing of 11~points.
% The word \textsc{Abstract} must be centered, in small caps, and in point size 12. Two
% line spaces precede the abstract. The abstract must be limited to one
% paragraph.

% Deep research is an advanced agentic capability that requires the systematic application of multi-agent technology to conduct complex research, including long-chain task decomposition and planning, as well as extensive search and reasoning across heterogeneous sources. A key challenge lies in effectively facilitate collaboration among multiple agents when tackling such complex tasks. In this paper, we propose InternAgent-DR, which redefines the collaboration paradigm of deep research multi-agent systems through a dynamic graph-driven planning strategy, endows InternAgent-DR with three key advantages: (i) improved logical reasoning capability, (ii) efficient context management, (iii) enhanced information integration across subtasks. InternAgent-DR demonstrates strong problem-solving capabilities in both general and scientific tasks, achieving state-of-the-art performance on GAIA and HLE, demonstrating its effectiveness for complex research scenarios and its potential in advancing scientific discovery.
% It is expected to contribute to advancements in scientific agents, particularly in areas such as therapeutic target discovery.

% (i) strenghened problem-solving logic through structured knowledge modeling, (ii) reduced contextual redundancy via per-node key information summarization, (iii) precise information transmission and composition through dynamic links across subtasks.

% Deep research (DR) is an inherently challenging task that demands both breadth and depth of thinking—exploring diverse knowledge spaces while reasoning through complex, multi-step dependencies. Addressing this dual requirement poses significant difficulties for traditional agentic systems. To address this, we propose InternAgent-DR(Deep Research), a multi-agent framework that leverages a dynamic thought graph to support wide exploration and deep reasoning. The thought graph enables breadth through parallel subtask expansion and depth via hierarchical decomposition and refinement. Crucially, by evaluating the outcomes of thought node executions, InternAgent-DR can dynamically revise its thought graph, refining its strategy based on new insights. This adaptive, graph-driven approach ensures precise information flow and efficient coordination among agents. InternAgent-DR achieves state-of-the-art performance on both general and scientific benchmarks, including GAIA and HLE, demonstrating its effectiveness for complex research scenarios and its promise in advancing scientific discovery.

% Deep research (DR) is an inherently challenging task that demands both breadth and depth of thinking—exploring diverse knowledge spaces while reasoning through complex, multi-step dependencies. Meeting these dual requirements poses significant difficulties for conventional agentic systems which function sequentially. To address this, we propose InternAgent-DR (Deep Research), a multi-agent framework that leverages a dynamic knowledge flow to support wide exploration and deep reasoning. The knowledge flow supports expansive exploration through parallel subtask expansion and enables deep reasoning via hierarchical decomposition and iterative refinement. Notably, InternAgent-DR dynamically adjusts its knowledge flow in response to real-time evaluations of thought node outcomes, allowing it to refine its strategy and adapt based on new insights. InternAgent-DR achieves state-of-the-art performance on both general and scientific benchmarks, including GAIA and HLE, demonstrating its effectiveness in complex research scenarios and its potential to advance scientific discovery.

%%%大概介绍经典deep research框架
%当前的深度研究智能体大致可以分为两类架构。第一类是单一 LLM 架构，由单个模型统筹整个研究过程，并调用多种工具，通常包括信息检索、网页探索和内容处理。在这种模式下，LLM 通过迭代地收集和分析信息、进行上下文感知的决策，并与动态的在线环境持续交互，从而生成全面的答案。然而，该方案对模型的理解能力要求较高，同时限制了系统整体的灵活性，不利于模块化扩展。第二类是多智能体系统，不同的 LLM 被赋予预定义的角色，通过协作实现与外部信息源的有效交互。在此类系统中，规划器负责制定执行计划，而专门的执行智能体则按照计划进行深入研究和问题解决。这种架构不仅能够更好地处理复杂研究任务，还显著增强了在通用场景下的灵活性与可扩展性，因此已被广泛应用于众多商用和开源的 deep research agent 框架中。

% Deep research agents can be broadly categorized into two architectural paradigms. The first is the single-LLM architecture, in which a single model orchestrates the entire research process while invoking a suite of tools, typically including information retrieval, web exploration, and content processing. In this setting, the LLM iteratively collects and analyzes information, makes context-aware decisions, and continuously interacts with dynamic online environments to generate comprehensive answers. However, this approach places high demands on the model’s reasoning capabilities, while limiting system flexibility and hindering modular extensibility. The second paradigm is the multi-agent system, where distinct LLMs are assigned predefined roles and collaborate to enable effective interaction with external information sources. Within such systems, a planner is always set for constructing execution plans, which are subsequently carried out by specialized execution agents to conduct in-depth research and problem solving. This design is particularly advantageous for handling complex research tasks, as it significantly enhances flexibility and scalability in general-purpose scenarios. Consequently, multi-agent architectures have been widely adopted in both commercial and open-source deep research agent frameworks. 

%%%研究背景，由llm切入deep research
%近年，大语言模型（LLMs）的快速发展显著推动了人工智能的发展和AI agent的进步。LLMs 展现出在文本生成、问答和知识推理等任务中的强大能力，并逐渐成为通用人工智能的重要基础。然而，尽管 LLMs 在已有知识的调用和语言表达方面表现优异，它们普遍缺乏面向开放环境的自主信息获取与深度研究能力。在真实的研究场景中，信息往往分散在动态变化的网络资源之中，研究者需要通过主动搜索、跨源比对以及与交互式工具的结合，才能形成系统而深入的结论。单纯依赖模型内部的参数化知识，难以满足这一需求。基于这一现实挑战，学界与工业界开始探索深度研究（Deep Research）Agent的范式，希望将 LLMs 的语言理解与推理能力与外部信息检索、工具调用和交互过程相结合，从而赋予模型更接近人类研究者的探索性与系统性。
% The rapid rise of large language models (LLMs) has advanced AI and accelerated the development of AI agents. While LLMs excel at text generation, question answering, and reasoning, they struggle to autonomously seek external information in open-world settings. To bridge this gap, Deep Research (DR) Agents like OpenAI-Deepresearch~\citep{openai2025deepresearch} and Perplexity~\citep{perplexity2025deepresearch}, which combine LLMs’ reasoning with retrieval, tool use, and interaction, enabling more systematic and exploratory research akin to humans.

%%%阐述现在多智能体架构的planner缺陷，引出我们的改进思路。
% 尽管多智能体架构具备较高的灵活性和可扩展性，但如何通过规划器（planner）制定合理的执行计划、有效管理执行过程中的上下文知识，以及协调多个智能体之间的协作，仍然是一个亟待解决的关键问题。目前的主流方案通常由规划器生成逐步的串行计划，并由执行器（executor）依次完成相应步骤。这种方式虽然能够较为直接地实现问题求解思路的规划，但也引发了两个突出挑战：其一，串行的执行流程对模型的上下文管理提出了严格要求，过长的上下文容易导致上下文窗口溢出；其二，缺乏对执行过程中的上下文知识结构的系统化规划与有效管理，可能导致推理结构与知识结构之间的不一致。在 WebShaper 中，作者提出了一种基于形式化驱动的知识检索范式（formalization-driven information seeking），通过引入形式化知识引导来确保推理逻辑的准确性与丰富性。这一思路也启发我们，利用形式化语言驱动机制有望提升深度研究智能体的规划能力。
% Although multi-agent architectures demonstrate high flexibility and scalability, critical challenges like coordinating collaboration among multiple agents remain unresolved. The mainstream approach today relies on the planner to generate a step-by-step serial plan. While this strategy provides a straightforward and effective way to organize problem-solving procedures, it introduces two major challenges. First, the serial execution process imposes strict requirements on context management, as excessively long contexts may lead to context window overflow. Second, the absence of systematic planning and effective management of contextual knowledge structures during execution can result in inconsistencies between reasoning structures and knowledge structures. In WebShaper, the authors propose a formalization-driven information-seeking paradigm, where the introduction of formalized knowledge guidance ensures both accuracy and richness in reasoning logic. Inspired by this, we introduce formalization–driven planner to enhance the planning capabilities of deep research agents.

%在这篇文章中，我们开发了一个形式化语言驱动的open deep research系统——Internagent-DR，他使用一个graph planner建立的graph来规划任务的执行步骤，其中，graph当中的节点用于表示需要解决的子问题或是需要寻找的关键概念，而edges代表不同子问题和概念之间的依赖关系。通过graph planner的引入，InternAgent-DR能够在构建执行计划的同时推理解决问题的知识结构以及涉及到的实体、概念之间的逻辑关系，这种逻辑关系不仅能够帮助模型更清晰准确的解决给定的问题，而且能够在执行过程中根据node的划分来实现对执行过程中的信息的总结，有效减少了problem solving过程当中的上下文的冗余。同时，节点间根据edges的依赖关系实现了定向的知识输入，能够缓解模型在过多的知识当中的confusion，从而提高子任务执行的成功率和准确性。
%在本文中，我们提出并开发了一种形式化语言驱动的开放深度研究系统——InternAgent-DR。该系统采用基于图规划器（graph planner）的方式来构建任务执行步骤的图结构，其中，图中的节点用于表示待解决的子问题或需要检索的关键概念，而边则刻画了不同子问题与概念之间的依赖关系。通过引入图规划器，InternAgent-DR 在生成执行计划的同时，还能够推理问题求解所需的知识结构，以及相关实体与概念之间的逻辑关系。这种逻辑结构不仅有助于模型更清晰、准确地解决给定问题，还能在执行过程中基于节点划分实现信息的阶段性总结，从而有效减少问题求解过程中的上下文冗余。同时，节点间依赖关系所引导的定向知识输入，也在一定程度上缓解了模型在面对海量知识时可能出现的混淆现象，从而提高了子任务执行的成功率与准确性。


% In this work, we present InternAgent-DR, a graph-driven open deep research agent, which employs a graph planner to construct a formalized execution graph, where nodes represent subproblems to be addressed or key concepts to be retrieved, and edges capture the dependency relationships among them. By leveraging this graph planner, InternAgent-DR not only generates a comprehensive plan for problem solving but also infers the underlying knowledge structure and the logical relations among the involved entities and concepts. This structured planning paradigm enables the model to approach problems with greater clarity and precision. Furthermore, the node-based decomposition supports intermediate summarization during execution, thereby reducing contextual redundancy throughout the problem-solving process. At the same time, the directed knowledge flow guided by edge dependencies mitigates potential confusion caused by excessive information, ultimately enhancing both the success rate and the accuracy of subtask execution.

%为了展示我们的InternAgent-DR的优越性能，我们在GAIA——一个考验AI assistants解决通用问题能力的榜单，以及高难度的科学问答榜单HLE和GPQA上验证了我们的性能，如图一所示，我们的InternAgent-DR在两种任务、三个benchmark上均达到了一流Deep research的性能，其中，GAIA、HLE上均达到了state of the art的水平，GPQA也实现了极高的水准。这些结果都说明我们的InternAgent-DR在graph plan的帮助下具有优秀的解决各种问题的能力。



%----------


% A high-quality initial Knowledge Flow is essential for systematic execution of complex research tasks. Generating a complete flow in a single step is challenging and may produce redundant or unstable structures. To address this, we propose a Flow Generation Loop, which incrementally expands the flow layer by layer. At each iteration, the planner adds only the new nodes and their dependency edges, progressively refining the flow while preserving logical consistency and controllability. This mechanism improves stability and quality, providing a reliable structured backbone for subsequent execution and information propagation.

% At each iteration \(t\), the planner inspects all newly added nodes in \(G_t\) to identify nodes that require further decomposition or additional information. For each such node \(v \in G_t\), the planner generates a set of successor nodes \(\{v'\}\), which may include sub-questions, intermediate reasoning steps, or evidence nodes. Dependency edges \((v' \rightarrow v)\) are then created to connect these new nodes to the existing graph, resulting in the updated knowledge flow:
